Learning Feature Descriptors for Pre- and Intra-operative Point Cloud Matching for Laparoscopic Liver Registration

Purpose: In laparoscopic liver surgery (LLS), pre-operative information can be overlaid onto the intra-operative scene by registering a 3D pre-operative model to the intra-operative partial surface reconstructed from the laparoscopic video. To assist with this task, we explore the use of learning-based feature descriptors, which, to our best knowledge, have not been explored for use in laparoscopic liver registration. Furthermore, a dataset to train and evaluate the use of learning-based descriptors does not exist. Methods: We present the LiverMatch dataset consisting of 16 preoperative models and their simulated intra-operative 3D surfaces. We also propose the LiverMatch network designed for this task, which outputs per-point feature descriptors, visibility scores, and matched points. Results: We compare the proposed LiverMatch network with anetwork closest to LiverMatch, and a histogram-based 3D descriptor on the testing split of the LiverMatch dataset, which includes two unseen pre-operative models and 1400 intra-operative surfaces. Results suggest that our LiverMatch network can predict more accurate and dense matches than the other two methods and can be seamlessly integrated with a RANSAC-ICP-based registration algorithm to achieve an accurate initial alignment. Conclusion: The use of learning-based feature descriptors in LLR is promising, as it can help achieve an accurate initial rigid alignment, which, in turn, serves as an initialization for subsequent non-rigid registration. We will release the dataset and code upon acceptance.

==> Table/ablation.tex <==
\begin{table*}[htpb]
\centering
\caption{Registration evaluation results and feature extraction time.}
    % and their running time.
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
& IR $\%$   & MR $\%$ \\ \hline
GCN &  32.72 $\pm$ 6.01    & 14.79 $\pm$ 3.58  \\ 
Without score & 31.46  $\pm$    6.04  &   13.83  $\pm$    3.53    \\
\hline
% Predator\cite{huang2021predator} &\multirow{2}{*}{N-ICP} & 0.0  $\pm$   0.0    \\
% LiverMatch    &    & 0.0 $\pm$ 0.0  \\
%  \hline
\end{tabular}
}
\label{tab:registration}
\end{table*}

   

==> draft.tex <==
\begin{document}

% Open-source\cite{fedorov2015open}
% It is widely hypothesized that image registration is an essential component in such systems.

% Therefore, a method that is robust to this potential variability, or that can handle missing data in regions where the prostate boundary is not clear, would be highly valuable, as mid-gland segmentation can be done robustly [11].

% we make both approaches available as open-source tools to facilitate development and evaluation of registration methodologies and to support clinical research in image-guided prostate interventions.

% Registration of signed distance maps with B-spline regularization.

% Biomechanically constrained surface registration

% Our registration tools implement novel registration approaches and produce acceptable registration results, aiming to reduce the barriers in development and deployment of interventional research solutions for prostate image-guided interventions and facilitate comparison with similar tools.

% Physics \cite{suwelack2014physics}

% The main reasons for this are soft-tissue
% deformations caused by, e.g., the pneumoperitoneum, surgical
% instruments, heartbeat, or respiratory motion. In order to accurately register planning data to the patient (and thus provide
% a meaningful guidance), these deformations have to be compensated. Intraoperative imaging such as stereo endoscopic,
% time-of-flight, or laser range scanner data can be used to obtain information about the surface of the moving tissue.11,21
% In this context, the intraoperative surface has to be matched
% to the preoperative model. The shape matching is especially
% challenging in the intraoperative setting due to noisy sensor
% data, only partially visible surfaces, and ambiguous shape descriptors.

% Shape matching (i.e., surface registration) is a classic problem in computer graphics, robotics, medical imaging, and related fields. Matching algorithms based on shape descriptors
% allow a robust rigid alignment of surfaces.10,20 For nonrigid
% shape matching, a dense set of corresponding feature points
% has to be found. Additionally, the global consistency of a nonrigid transformation is usually ensured by adding a regularization term to the minimization criterion.20 Different types
% of regularization such as geodesic distance, transformation
% similarity,20 and deformation based measures6,34 have been
% proposed in the literature. Gilles et al. enforce correspondence
% by projecting points on the target surface and connect corresponding pairs through springs.14,15 In this context, they use
% a deformation model that is based on blending closest rigid
% forms. Myronenko et al. treat the registration process as a
% probability density estimation problem.22 This approach called
% coherent point drift (CPD) algorithm was extended to include
% nonrigid matching by using a regularization term that ensures
% the smoothness of the deformation. For an extensive review of
% current rigid and nonrigid surface registration techniques, we
% refer to Tam et al.30


% Image deformation uses the relationship between surfaces that is identified during surface matching to deform the preoperative volume model. The internal
% tissue in the deformed volume model, such as tumors or
% vessels, is used to determine the location of intraoperative

% 1. align them in the same coordinate. 2. non-rigid registration. 3. image deformation.
% General pipeline and definition.
% initial registration
% The preoperative and intraoperative models use different
% imaging modalities or coordinate systems so pre-registration,
% which is also called initial registration, is necessary to ensure
% that both modalities align. This usually involves rigid transformation using a fast algorithm.

% There are two parts in image registration techniques: surface matching and image deformation. Surface matching
% determines the relationship between the intraoperative and preoperative surfaces. Image deformation uses the relationship between surfaces that is identified during surface matching to deform the preoperative volume model. The internal
% tissue in the deformed volume model, such as tumors or
% vessels, is used to determine the location of intraoperative

% The registration of intra-operative CT images to laparoscopic 2D images of the
% exploration video is defined as the initial registration problem. In the literature,there are three main approaches to this problem: manual alignment, automatic
% rigid registration and deformable registration. Manual alignment can be done
% by a specialist between the 3D pre-operative images and 2D intra-operative
% images. This solution is relevant only when considering small deformations
% with almost rigid organs. Moreover, a specialist in anatomy is needed during
% the procedure, and the result and time needed for the procedure are strongly
% operator-dependent. If the deformation is negligible, another solution is to
% search for the rigid transform that minimizes the distance between surface
% points of the transformed model and the target surface. Concretely, anatomical
% features can be used to initialize an ICP algorithm [4]. The algorithm may fail
% if the features used are hardly seen in the 2D images. For strong deformations,
% deformable registration has to be used. This is technically very challenging
% and involves organ-specific parameter tuning.
% \textbf{Challenges and our goals}
% tumors or vessels
% The shape matching is especially
% challenging in the intraoperative setting due to noisy sensor
% data, only partially visible surfaces, and ambiguous shape descriptors. 

% Shape matching (i.e., surface registration) is a classic problem in computer graphics, robotics, medical imaging, and related fields. Matching algorithms based on shape descriptors
% allow a robust rigid alignment of surfaces.10,20 For nonrigid
% shape matching, a dense set of corresponding feature points
% has to be found.

% We focus on the initial registration and surface registration part.


% For strong deformations,
% deformable registration has to be used. This is technically very challenging
% and involves organ-specific parameter tuning.

% Various pipelines have been proposed to solve the challenge problem. D

% the first step is to rigidly align them in the same coordinate, which can be done manually, semi-automatically\cite{plantefeve2016patient}, and automatically \cite{labrunie2022automatic,koo2022automatic}. Landmarks and contours are needed to be identified manually or automatically. In the second step, deformable/non-rigid registration methods are involved to match the intraoperative and preoperative surfaces.

% \begin{table}[t]
%     % \setlength{\tabcolsep}{4pt}
%     % \renewcommand{\arraystretch}{1.2}
% 	\centering
% 	\caption{Results. with different surface visible ratios.}
% 	\label{tab:big_predator}
% 	\resizebox{0.9\linewidth}{!}{
%     \begin{tabular}{lccccccc}
% 			\toprule
% 		    Mean disp. & $[0.2, 0.3]$ & $(0.3, 0.4]$ & $(0.4, 0.5]$ & $(0.5, 0.6]$ & $(0.6, 0.7]$ & $(0.7, 0.8]$ & $(0.8, 1.0]$ \\
%             \midrule
%  			& \multicolumn{7}{c}{\textit{CE}} \\
%  			\midrule
%  			Predator & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0   \\
%  			Lepard & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
%  			Method & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
%  			\midrule
%  			& \multicolumn{7}{c}{\textit{RE}} \\
%  			\midrule
%  			Predator & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0   \\
%  			Lepard & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
%  			Method & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
%  			\midrule
% %  			 \midrule
% %  			& \multicolumn{7}{c}{\textit{Inlier Ratio (\%), $\sigma=2mm$}} \\
% % 		    \midrule
% %  			3DSN & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0   \\
% %  			FCGF & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% %  			Method & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% %  			\midrule
% %  			& \multicolumn{7}{c}{\textit{Inlier Ratio (\%), $\sigma=3mm$}} \\
% % 		    \midrule
% %  			3DSN & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0   \\
% %  			FCGF & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% %  			Method & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% % 			\bottomrule
% 	\end{tabular}
% 	}
% \end{table}

% \begin{table}[t]
%     % \setlength{\tabcolsep}{4pt}
%     % \renewcommand{\arraystretch}{1.2}
% 	\centering
% 	\caption{Results. CE with different mean displacements.}
% 	\label{tab:big_predator}
% 	\resizebox{0.9\linewidth}{!}{
%     \begin{tabular}{lccccccc}
% 			\toprule
% 		    Mean disp. & $[0.2, 0.3]$ & $(0.3, 0.4]$ & $(0.4, 0.5]$ & $(0.5, 0.6]$ & $(0.6, 0.7]$ & $(0.7, 0.8]$ & $(0.8, 1.0]$ \\
%             \midrule
%  			& \multicolumn{7}{c}{\textit{CE}} \\
%  			\midrule
%  			Predator & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0   \\
%  			Lepard & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
%  			Method & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
%  			\midrule
%  			& \multicolumn{7}{c}{\textit{RE}} \\
%  			\midrule
%  			Predator & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0   \\
%  			Lepard & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
%  			Method & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
%  			\midrule
% %  			 \midrule
% %  			& \multicolumn{7}{c}{\textit{Inlier Ratio (\%), $\sigma=2mm$}} \\
% % 		    \midrule
% %  			3DSN & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0   \\
% %  			FCGF & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% %  			Method & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% %  			\midrule
% %  			& \multicolumn{7}{c}{\textit{Inlier Ratio (\%), $\sigma=3mm$}} \\
% % 		    \midrule
% %  			3DSN & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0   \\
% %  			FCGF & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% %  			Method & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
% % 			\bottomrule
% 	\end{tabular}
% 	}
% \end{table}



% $\mathbf{S} \in \mathbb{R}^{n\times3}$ and $\mathbf{T} \in \mathbb{R}^{m\times3}$ to superpoints $\mathbf{S}' \in \mathbb{R}^{n'\times3}$ and $\mathbf{T}' \in \mathbb{R}^{m'\times3}$, and extract their associated features $\mathbf{x}^{\mathbf{S}'} \in \mathbb{R}^{d \times n'}$ and $\mathbf{x}^{\mathbf{T}'} \in \mathbb{R}^{d \times m'}$. 

% the radius neighborhood of point

% $\mathbf{S} \in \mathbb{R}^{n\times3}$
% and $\mathbf{T} \in \mathbb{R}^{m\times3}$ are down sampled to $\mathbf{S}' \in \mathbb{R}^{n'\times3}$ and $\mathbf{T}' \in \mathbb{R}^{m'\times3}$

% . The encoder down sam

% to extract key-points from a raw point cloud and their associated features. 

% In the same encoder,

% In the shared encoder, a series of ResNet-like blocks and strided convolutions aggregate the raw points into \textit{superpoints} $\mathbf{P}'\in\mathbb{R}^{N'\times 3}$ and 
% $\mathbf{Q}'\in\mathbb{R}^{M'\times 3}$ with associated features $\mathbf{X}^{\mathbf{P}'} \in \mathbb{R}^{N{'} \times b}$ and $\mathbf{X}^{\mathbf{Q}'} \in \mathbb{R}^{M' \times b}$.
% Note that superpoints correspond to a fixed receptive field, so their number depends on the spatial extent of the input point cloud and may be different for the two inputs.

%The KPConv backbone has an Unet-like structure. The encoder extracts super-points

%The default KPFCN has an UNet-like
% structure with the same number of pooling/un-pooling layers in the encoder/decoder.

% of KPFCN backbone to extract 

% We follow [40] and first down-sample raw point clouds
% with a voxel-grid filter of size V , such that P and Q have
% reasonably uniform point density. In the shared encoder, a series of ResNet-like blocks and strided convolutions ag-gregate the raw points into superpoints P 0 ∈ R N ×3 and Q 0 ∈ R M ×3 with associated features X P ∈ R N ×b and
% X Q ∈ R M ×b . Note that superpoints correspond to a fixed
% receptive field, so their number depends on the spatial ex-
% tent of the input point cloud and may be different for the
% two inputs.

% We follow [2, 20] to adopt the Kernel Point Convolu-
% tion (KPConv) [40] backbone for feature extraction. The KPConv backbone uses a series of ResNet-like blocks and
% strided convolutions to transform each input point cloud
% into a reduced set of keypoints X̃ ∈ R M ×3 , Ỹ ∈ R N ×3
% and their associated features F X̃ ∈ R M ×D , F Ỹ ∈ R N ×D .
% In contrast to [2, 20] that subsequently perform upsampling
% to obtain feature descriptors of the original point cloud res-
% olution, our approach directly predicts the transformed key-
% point locations using the downsampled features.
% The default KPFCN \cite{thomas2019kpconv} has an UNet-like
% structure with the same number of pooling/un-pooling layers in the encoder/decoder.

% KPFCN backbone \cite{thomas2019kpconv}
% We build Φ based on the KPFCN backbone [62].
% KPFCN possesses the inductive bias of translation equivariance and locality, which are well suited for local geometry
% feature extraction. The default KPFCN has an UNet-like
% structure with the same number of pooling/un-pooling layers in the encoder/decoder. We remove the decoder units
% after the 2nd to the last un-pooling layer from the KPFCN
% backbone. Thus the output Sˆ and Tˆ are the down-sampled
% point clouds. 
% \subsubsection{Global Geometry Encoder}


% Given point clouds $\mathbf{S}$ and $\mathbf{T}$, the encoder extract super-points $\mathbf{S'}$ and $\mathbf{T'}$ along with their associated features $\mathbf{x}^{\mathbf{S}'}$ and $\mathbf{x}^{\mathbf{T}'}$. The features $\mathbf{x}^{\mathbf{S}'}$ and $\mathbf{x}^{\mathbf{T}'}$ only carry information from their close neighborhood points. To let a point interact with the points in the same point cloud, and the points in the other point cloud, the Transformer uses a self-attention layer and a cross-attention layer to update $\mathbf{x}^{\mathbf{S}'}$ and $\mathbf{x}^{\mathbf{T}'}$ with self-global geometry and cross-global geometry information. 

%\subsubsection{Local Geometry Encoder}

% The KPConv features from the previous step are linearly
% projected into a lower dimension d = 256. These projected
% features are then fed into L = 6 transformer cross-encoder 1
% layers. Each transformer cross-encoder layer has three sub-
% layers: 1) a multi-head self-attention layer operating on the
% two point clouds separately, 2) a multi-head cross-attention
% layer which updates the features using information from the
% other point cloud, and 3) a position-wise feed-forward net-
% work. The cross-attention enables the network to compare
% points from the two different point clouds, and the self-
% attention allows points to interact with other points within
% the same point cloud when predicting its own transformed
% position, e.g. using rigidity constraints. Note that the net-
% work weights are shared among the two point clouds but
% not among the layers.

% We adopt the single-head Transformer \cite{vaswani2017attention,li2022lepard} to encode self-global geometry and cross-global geometry information. The Transformer consists of a self-attention layer and a cross-attention layer.

% in the same point cloud, and the points in the other point cloud

% marked as $\mathbf{\hat{x}}^{\mathbf{S}'} \in \mathbb{R}^{n' \times d'}$ and $\mathbf{\hat{x}}^{\mathbf{T}'} \in \mathbb{R}^{m' \times d'}$.

% To feed a feature into a transformer, $\mathbf{x}^{\mathbf{S}'} \in \mathbb{R}^{n' \times d}$ and $\mathbf{x}^{\mathbf{T}'} \in \mathbb{R}^{m' \times d}$ are linearly projected into a new dimension $d'=256$. 

%The output feature dimension of a transformer is same as the input feature dimension. %We adopt the transformer implementation in \cite{li2022lepard} in this study.

% the same point cloud,
% Instead of calculating $\mathbf{q}$, $\mathbf{k}$, and $\mathbf{v}$ from the same point cloud,
% why self attention
% Complexity. Smooth.
% After the local geometry extraction, x Ŝ and x T̂ are
% passed through the transformer block with a self attention
% layer to aggregate the global context, followed by a cross
% attention layer to exchange information between two point
% clouds.
% local geometry feature extraction.
% So far, the features X P , X Q in the bottleneck encode
% 0
% the geometry and context of the two point clouds. But X P
% has no knowledge of point cloud Q and vice versa. In order
% to reason about their respective overlap regions, some cross-
% talk is necessary. We argue that it makes sense to add that
% cross-talk at the level of superpoints in the bottleneck, just
% like a human operator will first get a rough overview of the
% overall shape to determine likely overlap regions, and only
% after that identifies precise feature points in those regions.


\end{document}
